Populations of ultraluminous X-ray sources in galaxies: origin and evolution

Employing hybrid population synthesis, a model of the population of ultraluminous X-ray sources (ULX) in the binary systems with a black hole (BH) accretors is computed. It is compared to the model of the population of ULX with magnetized neutron stars (NS) that can be observed as pulsating ULX (Kuranov et al. 2020). A model of formation of BH is considered, in which their mass is determined by the mass of stellar CO core immediately before the collapse, as well as "delayed" and "rapid" collapse models (Fryer et al. 2012). Possible transiency of ULX due to accretion disks instability is taken into account The parameters and evolution of ULX are computed for the galaxies with constant star formation rate (SFR) and for the ones formed by an instantaneous star formation burst. The maximum number of ULX with BH ($\sim 10$) is reached in the galaxies with stationary $ SFR=10$\msun/yr in $\sim 1$ Gyr after beginning of star formation. ULX which are observed after the end of star formation, are binaries, in which BH and/or NS formed before the completion of star formation, while long-living donors with the mass $\sim$\msun\ continue RLOF or even fill their Roche lobes later. In several Gyr after completion of star formation the number of ULX in the galaxies with mass $M_G=10^{10}$\,\msun\ becomes less than 1 per 10 galaxies, most of them are ULX with NS. In ULX with NS, regardless of the adopted SFR model, dominate persistent sources with the donor overflowing Roche lobe. The number of transient sources is by more than an order of magnitude lower. Wind-accreting ULX are by an order of magnitude more rare than the sources with accretion via RLOF.

==> table2.tex <==
\begin{table}[t]
\vspace{6mm}
\begin{center}
\caption{Отношение численности \bux\ и \nux\ 
в модельной галактике c постоянной скоростью ЗО SFR=1\,\msun/год с возрастом  $t=10$ млрд. лет после начала ЗО в различных моделях формирования ЧД. }
\label{t:ratio}
\scalebox{0.72}{
%\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\begin{tabular}{c|c|c|c|}
\hline 
\hline 
%\hrule[-1ex]{0pt}{2.5ex} 
Model          &C265-05&C265-1&C265-4\\30-05&C30-1&C30-4&D265-05&D265-1&D265-4&D30-05&D30-1&D30-4&R265-1& R30-1 \\ 
\hline 
\rule[-1ex]{0pt}{2.5ex} $\frac{\bux}{\nux}$ &0.96   &1.89  &0.04 \\
Model          &30-05  & C30-1&C30-4  \\
\rule[-1ex]{0pt}{2.5ex} $\frac{\bux}{\nux}$ &2.51   &2.61  &0.04  \\
                 &0.67  &0.52 &0.04\\  
Model            &D265-05&D265-1&D265-4   \\
\rule[-1ex]{0pt}{2.5ex} $\frac{\bux}{\nux}$&0.07  &0.69 &0.07   &0.58&0.24 \\
Model  
\hline 
\hline
\end{tabular} 
}
\end{center}
\end{table}

